X-Align++: cross-modal cross-view alignment for Bird's-eye-view segmentation

Bird's-eye-view (BEV) grid is a typical representation of the perception of road components, e.g., drivable area, in autonomous driving. Most existing approaches rely on cameras only to perform segmentation in BEV space, which is fundamentally constrained by the absence of reliable depth information. The latest works leverage both camera and LiDAR modalities but suboptimally fuse their features using simple, concatenation-based mechanisms. In this paper, we address these problems by enhancing the alignment of the unimodal features in order to aid feature fusion, as well as enhancing the alignment between the cameras' perspective view (PV) and BEV representations. We propose X-Align, a novel end-to-end cross-modal and cross-view learning framework for BEV segmentation consisting of the following components: (i) a novel Cross-Modal Feature Alignment (X-FA) loss, (ii) an attention-based Cross-Modal Feature Fusion (X-FF) module to align multi-modal BEV features implicitly, and (iii) an auxiliary PV segmentation branch with Cross-View Segmentation Alignment (X-SA) losses to improve the PV-to-BEV transformation. We evaluate our proposed method across two commonly used benchmark datasets, i.e., nuScenes and KITTI-360. Notably, X-Align significantly outperforms the state-of-the-art by 3 absolute mIoU points on nuScenes. We also provide extensive ablation studies to demonstrate the effectiveness of the individual components.

==> include/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we present comprehensive performance evaluations of X-Align and compare it with baselines and the current state of the art. We further evaluate the benefits in performance v/s added complexity of the three X-FF blocks and finally show qualitative results.\par
%-------------------------------------------------
\input{tables/nuscenes_seg.tex}
\input{tables/kitti360}
%-------------------------------------------------
\subsection{Experimental Setup}
\vspace{-4pt}

\textbf{Datasets:} We evaluate performance on the large-scale nuScenes benchmark~\cite{caesar2020nuscenes}, which provides ground-truth annotations to support BEV segmentation. It contains 40,000 annotated keyframes captured by a 32-beam LiDAR scanner and six monocular cameras providing a $360^\circ$ field of view. Following the BEV map segmentation setup from~\cite{liu2022bevfusion}, we predict six semantic classes: drivable lanes, pedestrian crossings, walkways, stop lines, carparks, and lane dividers.
We further evaluate on KITTI-360~\cite{liao2022kitti}, a large-scale dataset with 83,000 annotated frames, including data collected using two fish-eye cameras and a perspective stereo camera. KITTI-360 does not provide dense ground-truth annotations for BEV segmentation. Hence, we use the BEV segmentation annotations from~\cite{gosala22panopticbev} as ground truth. These contain both static classes such as \textit{road} and \textit{sidewalk}, along with dynamic objects such as \textit{cars} and \textit{trucks}.\par
%-------------------------------------------------
\textbf{Evaluation Metrics:} For BEV map segmentation, our primary evaluation metric is the mean Intersection Over Union (mIoU). Because some classes may overlap, we apply binary segmentation separately to each class and choose the highest IoU over different thresholds. We then take the mean over all semantic classes to produce the mIoU. This evaluation protocol was proposed in~\cite{liu2022bevfusion}. We additionally use Panoptic Quality (PQ)~\cite{kirillov2019panoptic} on KITTI-360 when evaluating panoptic BEV segmentation. 

To evaluate performance on the 3D object detection task, we use the mean Average Precision (mAP) and the nuScenes Detection Score (NDS) metrics, as defined in~\cite{caesar2020nuscenes}.
%-------------------------------------------------

% \textbf{Network Architecture}: In X-Align, we have a separate pipeline for camera images and LiDAR points that are later fused into a final feature map for BEV prediction, as shown in Figure~\ref{fig:method_overview}. For Nuscenes, we build on top of the BEVFusion~\cite{liu2022bevfusion} framework to train our baseline network. We train our networks within the mmdetection3d\footnote{https://github.com/open-mmlab/mmdetection3d} framework. In our camera pipeline, the images are downsampled into a size of $256\times704$ before being passed through a Swin-T~\cite{liu2021swin} or ConvNext~\cite{liu2022convnext} backbone pretrained on ImageNet~\cite{russakovsky2015imagenet}. The intermediate features extracted from the camera are passed through a set of FPN~\cite{lin2017feature} layers to retain the salient low-level encoder features. We pass the FPN features to View-Transformers based on LSS~\cite{philion2020lift}. As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels, we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase\footnote{https://github.com/Qualcomm-AI-research/InverseForm}.

\textbf{Network Architecture and Training}: For evaluation on nuScenes, we build upon BEVFusion~\cite{liu2022bevfusion} for the baseline and train our networks within mmdetection3d~\cite{mmdet3d2020}.
In the camera branch, images are downsampled to 256$\times$704 before going into a Swin-T~\cite{liu2021swin} or ConvNeXt~\cite{liu2022convnext} backbone pretrained on ImageNet~\cite{russakovsky2015imagenet}. The extracted features are fed into several FPN~\cite{lin2017feature} layers and then through a PV-to-BEV transformation based on LSS~\cite{philion2020lift} to be mapped into the BEV space. 
In the LiDAR branch, we voxelize the points with a grid size of 0.1m and use a sparse convolution backbone~\cite{yan2018second} to extract the features, which are then flattened onto the BEV space. Given the camera and LiDAR features in BEV space, we utilize our proposed X-FF mechanism from Section~\ref{sec:feature_fusion} to fuse them. We use the self-attention module in our main results, providing the best accuracy-computation trade-off (see Fig.~\ref{fig:gmacs}). The fused features are fed into a BEV encoder and FPN layers similar to those in SECOND~\cite{yan2018second} and subsequently to a segmentation head as in BEVFusion~\cite{liu2022bevfusion}. Since nuScenes does not provide ground-truth PV segmentation labels, we utilize a SOTA model pre-trained on Cityscapes to generate pseudo-labels for supervising our PV segmentation in X-SA. Specifically, we use an HRNet-w48~\cite{wang2020deep} trained with InverseForm~\cite{borse2021inverseform}.

On KITTI-360, we take the camera-only PanopticBEV~\cite{gosala22panopticbev} as the baseline, which we retrain using the code and hyperparameters released by the authors.
Then, we include our two proposed X-SA losses on top of this baseline to generate the X-Align$_{\mathrm{view}}$ results on KITTI-360.

Additional hyperparameters and training details for all experiments can be found in the Appendix.
%------------------------------------------------- 
%\textbf{Training}
%To ensure optimal performance, we initialize our model with a Swin-T~\cite{liu2021swin} or ConvNext~\cite{liu2022convnext} backbone pretrained on ImageNet~\cite{russakovsky2015imagenet}. We then train our model in a full end-to-end manner, without freezing any weights, using a cyclic learning rate and an Adam~\cite{kingma2014adam} optimizer for 20 epochs with an initial learning rate of 1e-4. We apply both LiDAR and Image augmentations to the data. Following ~\cite{wang2021pointaugmenting}, we apply fading in the last five epochs to retain the original data distribution and improve model performance. Training X-Align with 8 A100s GPUs and a batch size of 12 on nuScenes takes approximately one day. Further details on the hyperparameters of our pipeline can be found in the supplementary.
%-------------------------------------------------    

\input{figs/method_overview/varying_gmacs}
\input{figs/qualitative/qualitative.tex}

\subsection{Quantitative Evaluation} 
\vspace{-4pt}
%-------------------------------------------------

%-------------------------------------------------
% \textbf{nuScenes Camera-Lidar fusion:} We compare X-Align to SOTA 3D perception models on the BEV map segmentation task, whereby X-Align gains an even higher performance boost. Following~\cite{zhou2022crossview}, we set up the model evaluation for each class independently on various classes as they may overlap (\eg, a car-parking area is also a drivable space) and choose the maximum IoU across different thresholds. Further, we evaluate in the region-bound of [-50m, 50m]$\times$[-50m, 50m] around the ego car following~\cite{philion2020lift, zhou2022crossview, xie2022m2bev, li2022bevformer, liu2022bevfusion}. X-Align achieves a new record mIoU of \textbf{65.7\%} on nuScenes BEV segmentation and boosts the performance of the BEV segmentation SOTA across all modalities and classes by \textbf{3\%} in mIoU. Due to its novel feature alignment strategy and supervision, it can significantly push the IoU performance of each segmentation class. All increases across segmentation classes can be seen in detail in Table \ref{tab:nuscenes_seg}.\par

\textbf{nuScenes Camera-LiDAR Fusion:} We report segmentation results based on camera-LiDAR fusion in the bottom section of Table~\ref{tab:nuscenes_seg}. We evaluate in the region-bound of [-50m, 50m]$\times$[-50m, 50m] around the ego car following the standard evluation procedure on nuScenes~\cite{philion2020lift, zhou2022crossview, xie2022m2bev, li2022bevformer, liu2022bevfusion}. 
We compare our complete method \textbf{X-Align}$_{\mathrm{all}}$ with existing SOTA approaches on BEV segmentation and see that X-Align significantly outperforms them. Specifically, X-Align achieves a new record mIoU of \textbf{65.7\%} on nuScenes BEV segmentation and consistently improves across all the classes, thanks to the proposed novel cross-modal and cross-view alignment strategies. We used the Self-Attention block illustrated in Figure~\ref{fig:method_detail1} as our preferred X-FF strategy, as it provided the optimal trade-off in Figure~\ref{fig:gmacs}. For this strategy, the computational overhead (\textbf{0.8\%}) and increase in latency (\textbf{2\%}) is minimal as observed in Table~\ref{tab:nuscenes_seg}. We further show the performance of X-Align but without using the more advanced fusion module, \textit{i.e.}, \textbf{X-Align}$_{\mathrm{losses}}$, in the second last row of Table~\ref{tab:nuscenes_seg}. X-Align still significantly outperforms existing methods even without introducing additional computational complexity during inference. 

% \textbf{nuScenes Camera-Only:} To prove the efficacy of our auxiliary camera segmentation branch and losses, we train an instance of X-Align using the camera branch only for BEV map segmentation. Camera-only X-Align achieves a record mIoU of \textbf{\%58} and beats the prior camera-only SOTA by \textbf{\%1.4} in the absolute score. It shows that features in the camera branch benefit from constrained alignment and, when aligned properly, can enhance the performance of all models significantly. For camera-only models, this comes at no extra cost in inference time.\par

\textbf{nuScenes Camera-Only:} To demonstrate the efficacy of our X-SA scheme, we evaluate an instance of X-Align, \textit{i.e.}, \textbf{X-Align}$_{\mathrm{view}}$, using only the camera branch for BEV map segmentation. The results and comparisons are shown in the top part of Table~\ref{tab:nuscenes_seg}. It can be seen that \textbf{X-Align}$_{\mathrm{view}}$ considerably outperforms the existing best performance, achieving a record mIoU of \textbf{58.0\%}, surpassing the prior camera-only SOTA by \textbf{1.4} points in mIoU. This shows the benefit of X-SA, which enhances the intermediate semantic features and the PV-to-BEV transformation without incurring computational overhead at inference.\par

\textbf{KITTI-360 Camera-Only:} We present additional camera-only results on KITTI-360 in Table~\ref{tab:kitti}, for the task of panoptic BEV segmentation. In this case, we use PanopticBEV~\cite{gosala22panopticbev} as our baseline. Additionally, we include our two novel X-SA losses to train our \textbf{X-Align}$_{\mathrm{view}}$ model.\footnote{The baseline scores are obtained by training PanopticBEV using the authors' code in \href{https://github.com/robot-learning-freiburg/PanopticBEV}{https://github.com/robot-learning-freiburg/PanopticBEV.}}  It can be seen that our proposed approach improves the baseline in terms of both mIoU and PQ scores. 

Overall, our proposed X-Align consistently improves upon the existing methods across modalities and classes on both nuScenes and KITTI-360, demonstrating the efficacy of our proposed X-FF, X-FA, and X-SA components.


%-------------------------------------------------
\input{figs/qualitative/supp_qualitative.tex}
%-------------------------------------------------

\subsection{Accuracy-Computation Analysis}
\vspace{-4pt}
In Fig.~\ref{fig:gmacs}, we report the accuracy-computation trade-off by utilizing our different X-FF fusion strategies, including self-attention, spatial-channel attention, and pose-driven deformable convolution (DCNv2). It can be seen that when using spatial-channel attention, we achieve the highest accuracy improvement at a higher computational cost, while pose-driven DCNv2 introduces the least amount of additional cost but provides less performance gain. Using self-attention, on the other hand, provides the best trade-off between performance and complexity.

We further compare by naively scaling up the complexity of the baseline fusion, \textit{eg.}, by adding more layers and channels in the convolution blocks, shown by the blue curve. It can be seen that the baseline's performance saturates, and all our proposed fusion methods achieve better trade-offs as compared to the baseline. This again verifies that the baseline fusion using simple concatenation and convolutions does not provide the suitable capacity for the model to align and aggregate multi-modal features.
%-------------------------------------------------
\subsection{Qualitative Results}
\vspace{-4pt}

% In Fig.~\ref{fig:qualitative}, we present a scene from the nuScenes dataset, showing both LiDAR and Camera inputs and comparing the output BEV segmentation map across different models. In this scene, the baseline mispredicts the building in the NW image as a road and labels it as such in the BEV segmentation output in Figure~\ref{fig:qualitative}-d. The building does not appear in the LiDAR scan; thus, the LiDAR has no way of correcting the camera projection later in the fusion. By adding the auxiliary camera branch only, the Cross View Segmentation Alignment Loss can mitigate this erroneous projection and correct this projection, as shown in the X-Align (X-SA only) model in Figure~\ref{fig:qualitative}-e. However, remnants of this erroneous projection are only removed when we apply an intelligent fusion strategy and add X-FA and X-FF to our model. By adding these to our model, we can see in Figure~\ref{fig:qualitative}-f that our full X-Align Model is able to project camera points to BEV accurately and align the two modalities such that these driving-critical faults can be avoided. For more visual examples, please refer to the supplementary.\par

In Figs.~\ref{fig:qualitative},~\ref{fig:qualitative_s1},~\ref{fig:qualitative_s2},~\ref{fig:qualitative_s3}, and~\ref{fig:qualitative_s4}, we present qualitative results on five sample test scenes from nuScenes, showing both LiDAR and camera inputs. We compare the BEV segmentation maps of different models, including the baseline, X-Align$_{\mathrm{view}}$ (only using the two X-SA losses), and the full X-Align, \textit{i.e.}, X-Align$_{\mathrm{all}}$.

For each of these figures, we present a scenario from the validation set in nuScenes: a) six camera inputs, b) LiDAR scan, c) ground-truth BEV segmentation map, d) baseline BEV segmentation, e) BEV segmentation using \textbf{X-Align}$_{\mathrm{view}}$, and d) BEV segmentation \textbf{X-Align}$_{\mathrm{all}}$. For each image, we observe that the baseline model prediction is highly erroneous in the region highlighted in \textcolor{green}{green}. We highlight this region of interest in the input views as well. By using the two X-SA losses, \textbf{X-Align}$_{\mathrm{view}}$ can already correct substantial errors in the baseline prediction, and the \textbf{X-Align}$_{\mathrm{all}}$ model further improves accuracy.\par
%-------------------------------------------------

\section{Ablation Studies}
\label{sec:ablation_all}
In this section, we perform various ablation studies to evaluate each component of the X-Align framework.
%-------------------------------------------------
\input{tables/ablation.tex}

\subsection{Studying the effect of each component in isolation}
\label{sec:ablation}
We conduct an ablation study on the different X-Align components and summarize our results in Table~\ref{tab:ablation}. We evaluate model variants using different combinations of our proposed novel losses, including Cross-Modal Feature Alignment (X-FA) loss and our Cross-View Segmentation Alignment (X-SA) comprised of our PV and PV2BEV losses. Additionally, we investigate the effect of our Cross-Modal Feature Fusion (X-FF). 

Our X-Align$_{\mathrm{view}}$ variant, leveraging both PV and PV2BEV losses, improves the mIoU from \textbf{62.7\%} to \textbf{64.1\%} when compared to the baseline. Specifically, the PV loss alone contributes to a 1-point mIoU improvement. When using the X-FA loss, we increase the baseline mIoU from \textbf{62.7\%} to \textbf{63.4\%}. Finally, adding all the losses together, our X-Align$_{\mathrm{losses}}$ variant boosts the mIoU score to \textbf{64.3\%}, significantly surpassing the baseline's mIoU. Notably, these improvements rely on new training losses and have no computational overhead during inference.
% It provides evidence that an implicit Perspective2BEV projection in the camera branch can learn better feature alignment with the lidar branch when constrained to predict the same target output as the fusion branch but only through the auxiliary camera branch. 

% On the other hand, only applying a better fusion strategy using the X-FF module without any other losses allows the model to gain a \textbf{+2.6\%} mIoU improvement over the baseline. This shows that using simple concatenation between the two modalities' BEV features fails to align the features accurately, propagating misaligned features throughout the BEV decoder pipeline and degrading the model's overall performance. Finally, combining all our contributions and adding the X-FF module to the X-Align$_{\mathrm{losses}}$ model creates the X-Align$_{\mathrm{all}}$ model, which holds the best performance of \textbf{65.7\%} mIoU (\textbf{+3\% } gain against the baseline's \textbf{62.7\%} mIoU). These ablations prove that each of our contributions adds a constraint to further the alignment of the two modalities and pushes the model's mIoU performance even higher.

Next, we study the effect of our X-FF module. Without any new losses, X-FF enables a 2.6-point mIoU improvement over the baseline (with a minor increase of computation, cf.~Table~\ref{tab:ablation} and Fig.~\ref{fig:gmacs}). This shows that simple concatenation is a key limitation in the baseline, which fails to fuse the camera and LiDAR features properly. Finally, using all our novel loss functions together with the X-FF module, we arrive at the full X-Align$_{\mathrm{all}}$ model, which achieves the overall best performance of \textbf{65.7\%} mIoU, significantly higher than the baseline's \textbf{ 62.7\%} mIoU. Our extensive ablation study results show that each of our proposed components in X-Align provides a meaningful contribution to improving the SOTA BEV segmentation performance.\par

%-------------------------------------------------
\subsection{Varying Backbones}

%-------------------------------------------------
\input{tables/supp_backbones}
%-------------------------------------------------
To verify the generalizability of our X-Align method, we present results for three different encoders, \textit{i.e.}, SWin-T, ConvneXt-T, and ConvneXt-S, in Table~\ref{tab:backbones}. For this ablation study, we choose our \textbf{X-Align}$_{\mathrm{view}}$ variant because this shows that a given model can be improved without adding additional computational complexity during inference. Compared to the current state-of-the-art result from BEVFusion~\cite{liu2022bevfusion}, we can improve their result from 62.7 to 64.1 in terms of mIoU. Similar improvements can be observed for our additionally investigated backbones ConvneXt-T and ConvneXt-S. These results show that our method generalizes well to different backbones without hyperparameter tuning.
%-------------------------------------------------
\subsection{Adaptability to Noise}

%-------------------------------------------------
\input{tables/supp_noise}
%-------------------------------------------------

Another interesting property of deep neural network-based methods is their susceptibility to input perturbations because it gives insights into their robustness in real environments. Therefore, we add Gaussian noise to the input camera images and observe how the performance degrades in Table~\ref{tab:noise}.  The noise is zero-mean normalized, and $\sigma$ in Table~\ref{tab:noise} is the standard deviation of the Gaussian noise. From the table, we can deduce two main observations: First, the performance of X-Align methods under input perturbations is relatively stable compared to the baseline. We attribute this to the fact that the input camera noise will make the extracted camera feature less reliable. Due to our robust attention-based cross-modal feature fusion (X-FF), the method can still correct the camera features using LiDAR predictions. Our second interesting observation concerns the comparison to the baseline BEVFusion. We observe that our performance loss at a higher noise-variance is much smaller than for BEVFusion, e.g., the performance of our method \textbf{X-Align}$_{\mathrm{all}}$ at $\sigma=0.1$ drops from 65.7 to 59.6. In contrast, BEVFusion drops from 62.7 to 48.9. This shows superior properties of our method in terms of robustness.\par
%-------------------------------------------------
\subsection{Adverse Weather Conditions}

%-------------------------------------------------
\input{tables/supp_splits}
%-------------------------------------------------

To further investigate our method's robustness, we show results of how our method performs in adverse weather conditions in Table~\ref{tab:splits}. For this experiment, we use the metadata provided by nuScenes, which indicates the weather and light conditions of the recorded scene. With this information, we filter the validation set to obtain two splits containing all images recorded at night and all images recorded during rainy conditions. Our results show consistent improvement in these adverse conditions by \textbf{X-Align}$_{\mathrm{view}}$ as well as \textbf{X-Align}$_{\mathrm{all}}$. This shows that our method improves on comparably easy samples and difficult ones, which is an important property for future deployment of our method.
%-------------------------------------------------

\subsection{Extending the results to Camera and Radar Object Detection}

%-------------------------------------------------
\input{tables/nuscenes_det}
%-------------------------------------------------

To investigate if our proposed X-FF strategies can extend to other tasks beyond segmentation, we show results on Camera and Radar Fusion for 3D Object Detetion(3DOD). For this experiment, we first train a baseline model using on Camera and Radar inputs and fusing them using the vanilla convolution based fusion strategy from BEVFusion. We follow the baseline hyperparameters from BEVFusion for their 3DOD variant, and replace the LiDAR inputs with Radar inputs. We compare this baseline with our pose-driven deformable convolution, \textbf{X-FF}$_{\mathrm{pose}}$ described in Section~\ref{sec:feature_fusion}. We observe an improvement of \textbf{1.1} points on NDS and \textbf{0.8} points on mAP.    
%----------------------------------

==> include/instructions.tex <==
The ABSTRACT is to be in fully-justified italicized text, at the top
of the left-hand column, below the author and affiliation
information. Use the word ``Abstract'' as the title, in 12-point
Times, boldface type, centered relative to the column, initially
capitalized. The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous WACV abstracts to get a feel for style and length.

\section{Introduction}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the WACV 2023 web page
(\url{http://wacv2023.thecvf.com/submission/})
for a discussion of the policy on dual submissions.

\subsection{Paper length}
Papers must be no longer than eight pages, not including references.
Any pages in excess of eight pages must contain ONLY references ---
no text, figures, acknowledgements, tables, etc.

{\bf There will be no extra page charges for WACV 2023.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the \verb'\wacvfinalcopy' command in the document preamble.)  Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $087.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.


\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  In addition, in means you are extremely careful if you
share URLs to source code, github repositories, project websites,
datasets, etc. The URL or other information (e.g. your github user ID)
may identify you and would violate the anonymization policy.


For example, saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors20} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2020 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors20b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the WACV 70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double blind review policy, you can report results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors20} to
\cite{Alpher02,Alpher03,Authors20}.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.

Page numbers should be in footer with page numbers, centered and .75
inches from the bottom of the page and make it start at the correct page
number rather than the 9876 in the example.  To do this find the secounter
line (around line 33 in this file) and update the page number as
\begin{verbatim}
\setcounter{page}{123}
\end{verbatim}
where the number 123 is your assigned starting page.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors20}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
  \begin{center}
    {\small{
\begin{tabular}{llr}
\toprule
Method & Frobnability & Accuracy \\
\midrule
Theirs & Frumpy & 30.2\%\\
Yours & Frobbly & 45.2\%\\
Ours & Makes one's heart Frob & 99.9\%\\
\bottomrule
\end{tabular}
}}
\end{center}
\caption{Results.   Ours are better. If you prefer, you can put table
captions on top of the tables instead of on the bottom.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the WACV 2023 web page 
(\url{http://wacv2023.thecvf.com/submission/})
for a discussion of the use of color in your document.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: 
\url{https://www.computer.org/about/contact}.

==> include/intro.tex <==
\vspace{-8pt}
\section{Introduction}
\vspace{-2pt}

%-------------------------------------------------
\input{figs/contribution/contribution.tex}
%-------------------------------------------------
Bird's-eye-view (BEV) segmentation aims at classifying each cell in a BEV grid around the ego position. As such, it is a key enabler for applications like autonomous driving and robotics. For instance, the BEV segmentation map is a prerequisite for current works on behavior prediction and trajectory planning~\cite{hu2021fiery, tacs2016functional, wu2020motionnet}. It is also an important input modality for learning end-to-end controls (e.g., speed control, steering) in autonomous driving~\cite{chitta2021neat}.\par

Given the ubiquity of camera sensors, existing BEV segmentation methods predominantly focus on predicting BEV segmentation maps from camera images \cite{philion2020lift, xie2022m2bev, xu2022cobevt, zhou2022crossview}. However, the lack of reliable 3D information significantly limits the performance of these methods. A possible way to resolve this challenge is to leverage a LiDAR sensor and fuse the measured sparse geometric information with that contained in camera images. While camera-LiDAR fusion has been extensively studied for the task of 3D object detection, such fusion strategies are relatively unexplored for BEV segmentation. The concurrent work of~\cite{liu2022bevfusion} provides the first baseline using a simple concatenation of LiDAR BEV features and camera features projected from perspective view (PV) to BEV via estimated depth and voxel pooling. However, the PV-to-BEV projection can be inaccurate due to errors in depth estimation. As a result, in the concatenation stage, the network may aggregate poorly aligned features across the camera and the LiDAR branches, resulting in suboptimal fusion results.\par

In this paper, we propose a novel \textit{cross-modal, cross-view alignment strategy, X-Align}, which enforces feature alignment across features extracted from the camera and LiDAR inputs as well as segmentation consistency across PV and BEV to improve the overall BEV segmentation accuracy (cf.~Fig.~\ref{fig:contribution}). First, we propose a Cross-Modal Feature Alignment (X-FA) loss function that promotes the correlation between projected camera features and LiDAR features, as measured by cosine similarity. In addition, we incorporate attention to the Cross-Modal Feature Fusion (X-FF) of these two sets of modality-specific features instead of using simple concatenation as in~\cite{liu2022bevfusion}. This gives the network a more substantial capability to properly align and aggregate features from the two sensing modalities.\par

We further impose Cross-View Segmentation Alignment (X-SA) losses during training. We introduce a trainable segmentation decoder based on the intermediate PV camera features to generate PV segmentation. Next, we utilize the same PV-to-BEV transformation~\cite{philion2020lift} that converts PV camera features to BEV to convert the PV segmentation map into a BEV segmentation map, which is then supervised by the ground truth. We also supervise the intermediate PV segmentation map using pseudo-labels generated by a high-quality, off-the-shelf semantic segmentation model. In this way, the camera branch learns to derive intermediate features containing useful PV semantic features, providing richer information for BEV segmentation after being projected to BEV space. Moreover, this provides additional supervision on the PV-to-BEV module, allowing it to learn a more accurate transformation.\par

Our main contributions are summarized as follows:
\begin{itemize}
\setlength\itemsep{0pt}
    \item We propose a novel framework, X-Align, that enables better feature alignment and fusion across camera and LiDAR modalities and enforces segmentation alignment across perspective view and bird's eye view.  
    \item Specifically, we propose a Cross-Modal Feature Alignment (X-FA) loss to enhance the correlation between the camera and LiDAR features. We also devise an attention-based Cross-Modal Feature Fusion (X-FF).
    \item We further propose to enforce Cross-View Segmentation Alignment (X-SA) across the perspective view and bird's eye view, which encourages the model to learn richer semantic features and a more accurate PV-to-BEV projection.
    \item We conduct extensive experiments on the nuScenes and KITTI-360 datasets with comprehensive ablation studies that demonstrate the efficacy of X-Align. In particular, on nuScenes, we surpass the state-of-the-art in BEV segmentation by 3 absolute mIoU points.
\end{itemize}
%-------------------------------------------------------------------------

==> include/method.tex <==
% \section{X-Align: Cross-modal BEV Segmentation}
\section{Proposed X-Align Framework}
\vspace{-2pt}
%-------------------------------------------------------
\input{figs/method_overview/method_overview.tex}
%-------------------------------------------------------

This section describes X-Align, our novel cross-modal and cross-view alignment strategy. We first formally introduce the problem and describe a baseline method in Section~\ref{sec:method_formulation}. We provide an overview of X-Align in Section~\ref{sec:method_overview} and then discuss its components in detail, including Cross-Modal Feature Fusion (X-FF), Cross-Modal Feature Alignment (X-FA), and Cross-View Segmentation Alignment (X-SA) in Sections~\ref{sec:feature_fusion}, \ref{sec:feature_alignment}, \ref{sec:segmentation_alignment}, respectively. \par

\subsection{Problem Formulation and Baseline}\label{sec:method_formulation}
\vspace{-4pt}

% \textbf{Input and output definition}
Our goal is to develop a framework taking multi-modal sensor data $\mathcal{X}$ as input and predicting a BEV segmentation map $\hat{\bm{m}}\in\mathcal{S}^{H^{\mathrm{BEV}}\times W^{\mathrm{BEV}}}$, with resolution $H^{\mathrm{BEV}}\times W^{\mathrm{BEV}}$, and the set of classes $\mathcal{S}=\left\lbrace0, 1, \dots, \|\mathcal{S}\| \right\rbrace$. As illustrated in Fig.~\ref{fig:method_overview}, the set of inputs, $\mathcal{X} = \left\lbrace\bm{x}, \bm{l}\right\rbrace$, contains RGB camera images in PV, $\bm{x}\in\mathbb{R}^{N^{\mathrm{cam}}\times H^{\mathrm{cam}}\times W^{\mathrm{cam}}\times 3}$, where $N^{\mathrm{cam}}$, $H^{\mathrm{cam}}$, $W^{\mathrm{cam}}$ denote number of cameras, image height, and image width, respectively, as well as a LiDAR point cloud, $\bm{l}\in\mathbb{R}^{P\times 5}$, with number of points $P$. Each point consists of its 3-dimensional coordinates, reflectivity, and ring index. 
% Our method outputs either a BEV segmentation map $\bm{m}\in\mathcal{S}^{H^{\mathrm{map}}\times W^{\mathrm{map}}}$ with resolution $H^{\mathrm{map}}\times W^{\mathrm{map}}$ and the set of classes $\mathcal{S}=\left\lbrace0, 1, \dots, |\mathcal{S}| \right\rbrace$, or 3D bounding boxes $\bm{b}\in\mathbb{R}^{B\times 10}$ with maximum number of predicted bounding boxes $B$. Each bounding box contains three values for spatial extent, three for the position, two for velocity, as well as one for the yaw (\ie, box orientation), and one for the objectness score. Accordingly, $\mathcal{Y} = \left\lbrace \bm{m}, \bm{b}\right\rbrace$ or any subset thereof, depending on the desired tasks.
\par 
\textbf{Baseline Method}:
We first establish a baseline method of fusion-based BEV segmentation based on BEVFusion~\cite{liu2022bevfusion}.
% , which uses recent state-of-the-art architectures for 3D object detection. 
As shown in Fig.~\ref{fig:method_overview}, initial features are extracted from both sensor inputs. For camera images, a camera encoder, $\bm{E}^{\mathrm{cam}}$, extracts features in PV, $\bm{f}^{\mathrm{cam}}$. Subsequently, we use a feature pyramid network (FPN) and a PV-to-BEV transformation based on~\cite{philion2020lift} to obtain camera features in BEV space, following BEVDet~\cite{huang2021bevdet}. For the LiDAR points, we follow SECOND~\cite{yan2018second} in using voxelization and a sparse LiDAR encoder, $\bm{E}^{\mathrm{LiDAR}}$. The LiDAR features are projected to BEV space using a flattening operation as in~\cite{liu2022bevfusion}. 

These operations result in two sets of modality-specific BEV features, $\bm{\Tilde{f}}^{\mathrm{cam}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{cam}}}$ and $\bm{\Tilde{f}}^{\mathrm{LiDAR}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{LiDAR}}}$, with BEV space feature resolution $H^{\mathrm{lat}}\times W^{\mathrm{lat}}$ and number of channels $C^{\mathrm{cam}}$ and $C^{\mathrm{LiDAR}}$ for camera and LiDAR features, respectively. The features are then combined (e.g., by simple concatenation as in~\cite{li2021hdmapnet, liu2022bevfusion, harley2022simple}), resulting in fused features $\bm{\Tilde{f}}^{\mathrm{fused}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{fused}}}$, which are further processed by a BEV Encoder and FPN as in SECOND~\cite{yan2018second}. Finally, the features are processed by a segmentation head with the same architecture as in~\cite{liu2022bevfusion} to ensure comparability. This baseline model is trained using the focal cross-entropy loss~\cite{lin2017focal}:
\begin{equation}
    \mathcal{L}^{\mathrm{BEV}} = \mathrm{FocalCE}\left (\hat{\bm{y}}^{\mathrm{BEV}}, \bm{y}^{\mathrm{BEV}}\right), 
    \label{eq:focal_bev}
\end{equation}
where $\hat{\bm{y}}^{\mathrm{BEV}}\in\mathbb{R}^{H^{\mathrm{BEV}}\times W^{\mathrm{BEV}}\times S}$ are class probabilities and $\bm{y}^{\mathrm{BEV}}\in \left\lbrace 0,1\right\rbrace^{H^{\mathrm{BEV}}\times W^{\mathrm{BEV}}\times S}$ denotes the one-hot encoded ground truth. We can obtain the final classes $\hat{\bm{m}}$ by a pixel-wise argmax operation on $\hat{\bm{y}}$ during inference.\par

%-------------------------------------------------
\subsection{X-Align Overview}\label{sec:method_overview}
\vspace{-4pt}

% \textbf{X-Align Method Optimization}:
Building on top of the previously described baseline, we present our novel cross-modal and cross-view alignment strategy, X-Align (highlighted by red boxes in Fig.~\ref{fig:method_overview}). First, we improve the simple concatenation-based fusion with a Cross-Modal Feature Fusion (X-FF) module, which leverages attention and mitigates misalignment between features across modalities (Section~\ref{sec:feature_fusion}). Secondly, we propose a Cross-Modal Feature Alignment (X-FA) loss, $\mathcal{L}^{\mathrm{X\text{-}FA}}$, which promotes the correlation between features across modalities (Section~\ref{sec:feature_alignment}). Finally, we propose losses to enforce Cross-View Segmentation Alignment (X-SA) in Section~\ref{sec:segmentation_alignment}, where we supervise a PV segmentation predicted from the intermediate camera features with a loss $\mathcal{L}^{\mathrm{PV}}$ and the PV-to-BEV-projected version of this segmentation with a loss $\mathcal{L}^{\mathrm{PV2BEV}}$. These two losses provide more direct training signals to the PV-to-BEV transformation and encourage richer semantic features in PV before the transformation. Overall, our total optimization objective is
\begin{equation}
    \mathcal{L}^{\mathrm{X\text{-}Align}}\! =\! \lambda_1 \mathcal{L}^{\mathrm{BEV}}\! +\! \lambda_2 \mathcal{L}^{\mathrm{X\text{-}FA}}\! +\! \lambda_3 \mathcal{L}^{\mathrm{PV}}\! +\! \lambda_4 \mathcal{L}^{\mathrm{PV2BEV}},
\label{eq:final_loss}
\end{equation}
where $\lambda_{i},\, i\in\left\lbrace 1,2,3,4 \right\rbrace$ are the loss weighting factors.

%-------------------------------------------------
\subsection{Cross-Modal Feature Fusion (X-FF)}
\label{sec:feature_fusion}
\vspace{-4pt}
%-------------------------------------------------
In recent BEV segmentation literature~\cite{liu2022bevfusion, li2021hdmapnet, harley2022simple}, it is a common approach to utilize concatenation followed by convolution to combine features from multi-modal inputs, $\bm{\tilde{f}}^{\mathrm{cam}}$ and $\bm{\tilde{f}}^{\mathrm{LiDAR}}$, resulting in the aggregated features $\bm{\tilde{f}}^{\mathrm{fused}}$. However, the lack of reliable depth information can cause inaccurate PV-to-BEV transformation of features, which subsequently results in suboptimal alignment and fusion of multi-modal features. The convolution blocks utilized in existing approaches~\cite{liu2022bevfusion, li2021hdmapnet, harley2022simple} cannot rectify such misalignment due to their translation invariance. To address this issue, we propose more powerful, Cross-Modal Feature Fusion (X-FF) modules that can account for pixel-wise misalignment, as shown in Fig.~\ref{fig:method_detail1}. Next, we describe in detail our three proposed fusion designs.\par

\textbf{Self-Attention:} Our proposed X-FF using self-attention is shown in Fig.~\ref{fig:method_detail1} (left). We first stack features $\bm{\Tilde{f}}^{\mathrm{cam}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{cam}}}$ and $\bm{\Tilde{f}}^{\mathrm{LiDAR}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{LiDAR}}}$, and tokenize them into $K\times K$ patches with an embedding dimension of $L^{\mathrm{embed}}$. These patches are fed into a multi-head self-attention module~\cite{vaswani2017attention}. The output is then projected back to the original resolution using a deconvolution block, resulting in the final fused features $\bm{\Tilde{f}}^{\mathrm{fused}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{fused}}}$. By using self-attention, our proposed module can correspond to the camera and LiDAR features spatially, accounting for potential misalignment.\par
%-------------------------------------------------
\input{figs/method_details/method_detail1.tex}
%-------------------------------------------------
\textbf{Spatial-Channel Attention:} In this option, we leverage the recently proposed Split-Depth Transpose Attention (SDTA)~\cite{maaz2022edgenext}, as shown in Fig.~\ref{fig:method_detail1} (middle). It first performs spatial and channel mixing of the stacked camera and LiDAR features via depth-wise and point-wise convolutions. Then, it applies channel attention followed by a lightweight MLP. The output is passed through a deconvolution block to generate the fused features $\bm{\Tilde{f}}^{\mathrm{fused}}$. Spatial and channel mixing together with channel attention provides powerful capacity for the module to better address the misalignment between the camera and LiDAR features.\par 
%-------------------------------------------------
\textbf{Pose-Driven Deformable Convolution:} This design is illustrated in Fig.~\ref{fig:method_detail1} (right). We know that the transformation between modalities is a function of their relative poses to the ego vehicle. Hence, we apply an adaptive transformation, i.e., Deformable Convolution (DCNv2)~\cite{zhu2019deformable}, to the stacked multi-modal features $\bm{\Tilde{f}}^{\mathrm{cam}}$ and $\bm{\Tilde{f}}^{\mathrm{LiDAR}}$, which can implicitly learn the cross-modal alignment based on available pose information. More specifically, we process the pose matrices with an MLP to generate a pose embedding $\bm{\Tilde{f}}^{\mathrm{pose}}\in \mathbb{R}^{H^{\mathrm{lat}}\times W^{\mathrm{lat}}\times C^{\mathrm{pose}}}$, which is then concatenated with $\bm{\Tilde{f}}^{\mathrm{cam}}$ and $\bm{\Tilde{f}}^{\mathrm{LiDAR}}$. They are used to generate $K\times K$ offset vectors to be used by the DCNv2 block, which produces the output fused features $\bm{\Tilde{f}}^{\mathrm{fused}}$. \par
%-------------------------------------------------
% Our proposed X-FF blocks change the baseline network architecture and hence, vary the computational complexity of our network. In Section~\ref{sec:ablation}, we investigate this variation in computational complexity by demonstrating the effect of each block on the networks performance while observing the change in GFlops. We then compare this to simply varying the baseline network complexity and observing its performance at every scale.

Our proposed X-FF designs provide the network with the suitable capacity to properly align and fuse multi-modal features. While they introduce additional computations, they show more superior accuracy-efficiency trade-offs as compared to naively increasing the complexity of the baseline network, as we shall see in our study in Section~\ref{sec:ablation}.
%-------------------------------------------------
\subsection{Cross-Modal Feature Alignment (X-FA)}
\label{sec:feature_alignment}
\vspace{-4pt}

While our proposed X-FF modules can improve feature alignment, they incur additional computations, which may not always be feasible. As such, we propose a second measure to improve feature alignment with a Cross-Modal Feature Alignment (X-FA) loss $\mathcal{L}^{\mathrm{X\text{-}FA}}$ that is only applied during training and does not introduce additional computations for inference. It can also be used in conjunction with X-FF.\par 

Consider extracted features in BEV space, $\bm{\Tilde{f}}^{\mathrm{cam}}$ and $\bm{\Tilde{f}}^{\mathrm{LiDAR}}$, from camera and LiDAR branches, respectively. We promote the correlation between the two sets of features by imposing a cosine similarity loss between them:
\begin{equation}
    \mathcal{L}^{\mathrm{X\text{-}FA}} = \mathrm{CosineSim}\left (\bm{\Tilde{f}}^{\mathrm{cam}}, \bm{\Tilde{f}}^{\mathrm{LiDAR}}\right). 
    \label{eq:feature_alignment}
\end{equation}

%-------------------------------------------------
In order to apply this loss, there are two requirements. First, the camera features $\bm{\Tilde{f}}^{\mathrm{cam}}$ and LiDAR features $\bm{\Tilde{f}}^{\mathrm{LiDAR}}$ in BEV space need to have the same resolution. In this work, we ensure that the network parameters are chosen accordingly. In case both features have different resolutions, differentiable grid sampling~\cite{jaderberg2015spatial} can be used. Second, the channels $C^{\mathrm{cam}}$ and $C^{\mathrm{LiDAR}}$ should match for Eq.~(\ref{eq:feature_alignment}) to be applicable. This, however, is generally not the case. As such, we take all features from the lower-dimensional branch and enforce their similarity to several subsets of features from the higher-dimensional branch.


%-------------------------------------------------
\subsection{Cross-View Segmentation Alignment (X-SA)}
\label{sec:segmentation_alignment}
\vspace{-4pt}

In addition to encouraging feature alignment, we also impose alignment at the output segmentation level across PV and BEV using our Cross-Modal Segmentation Alignment (X-SA) losses. More specifically, for the camera branch, we take intermediate PV features and feed them through an additional decoder to generate a PV segmentation prediction $\hat{\bm{y}}^{\mathrm{PV}}\in\mathbb{R}^{N^{\mathrm{cam}}\times H^{\mathrm{cam}}\times W^{\mathrm{cam}}\times\|\mathcal{S}\|}$ (cf.~Fig.~\ref{fig:method_overview}, top part). We further transform $\hat{\bm{y}}^{\mathrm{PV}}$ to BEV space by utilizing the PV-to-BEV transformation as for the features, resulting in a projected BEV segmentation map $\hat{\bm{y}}^{\mathrm{PV} \rightarrow \mathrm{BEV}}\in\mathbb{R}^{H^{\mathrm{BEV}}\times W^{\mathrm{BEV}}\times \|\mathcal{S}\|}$. The projected BEV segmentation map is supervised w.r.t ground-truth BEV segmentation using a focal cross-entropy loss:
\begin{equation}
    \mathcal{L}^{\mathrm{PV2BEV}} = \mathrm{FocalCE}\left (\hat{\bm{y}}^{\mathrm{PV} \rightarrow \mathrm{BEV}}, \bm{y}^{\mathrm{BEV}}\right). 
\end{equation}

As for the PV segmentation, since PV ground truth is not always available on BEV perception datasets, we supervise it with a focal loss using pseudo-labels generated by a state-of-the-art model pretrained on Cityscapes~\cite{cordts2016cityscapes}, as follows:
\begin{equation}
    \mathcal{L}^{\mathrm{PV}} = \mathrm{FocalCE}\left (\hat{\bm{y}}^{\mathrm{PV}}, \bm{y}^{\mathrm{PV}}\right), 
\end{equation}

By introducing these two additional supervisions, we enforce that across PV and BEV, the segmentations are accurate and aligned through the PV-to-BEV transformation. This benefit is two-fold: First, the module used here is given by the same PV-to-BEV transformation as on the feature level in the main camera branch. Our X-SA loss provides additional supervision to more accurately train this key module. Second, imposing a PV segmentation loss $\mathcal{L}^{\mathrm{PV}}$ encourages the network to learn useful PV semantic features, providing richer semantic information for the downstream BEV features. Our X-SA components, including the additional decoder and the losses, are only used during training and do not require overhead at test time.\par

In summary, our complete X-Align framework \textbf{X-Align}$_{\mathrm{all}}$
proposes four additions to the baseline: the X-FF feature fusion module, along with three additional training losses: $\mathcal{L}^{\mathrm{X\text{-}FA}}$, $\mathcal{L}^{\mathrm{PV}}$, and $\mathcal{L}^{\mathrm{PV2BEV}}$. In cases where the network only takes camera inputs, we apply the two X-SA losses, $\mathcal{L}^{\mathrm{PV}}$ and $\mathcal{L}^{\mathrm{PV2BEV}}$, giving us the \textbf{X-Align}$_{\mathrm{view}}$ variant. In addition, in case extra computation is not allowed, we apply all three X-Align losses when training the network, forming the \textbf{X-Align}$_{\mathrm{losses}}$ variant. We extensively evaluate these variants as well as combinations of our proposed X-Align components in Section~\ref{sec:ablation}.

%-------------------------------------------------

==> include/related_work.tex <==
\section{Related Work}
 \vspace{-2pt}

\textbf{BEV Segmentation}:
The task of BEV segmentation has mostly been explored using (multiple) camera images as input. Building on top of Perspective View (PV) segmentation~\cite{borse2021inverseform, borse2021hs3, borse2022panoptic, zhang2022auxadapt, borse2023dejavu, hu2022learning, zhang2022perceptual}, early works used the homography transformation to convert camera images to BEV, subsequently estimating the segmentation map~\cite{abbas2019geometric, garnett2019lanenet, loukkal2021driving, zhu2021monocular}. As the homography transformation introduces strong artifacts, subsequent works moved towards depth estimation and voxelization~\cite{philion2020lift, roddick2018orthographic} for the PV-to-BEV transformation as end-to-end learning~\cite{lu2019monocular, roddick2020predicting}. This basic setup has been further explored in various directions: VPN~\cite{pan2020cross} explores domain adaptation, BEVerse~\cite{zhang2022beverse} and M\textsuperscript{2}BEV~\cite{xie2022m2bev} explore multi-task learning with 3D object detection, CoBEVT~\cite{xu2022cobevt} explores fusion of features from vehicles, Gosala \textit{et al}. explore panoptic BEV segmentation~\cite{gosala22panopticbev}, while several works explore incorporation of temporal context~\cite{hu2021fiery, saha2021enabling}. Furthermore, CVT~\cite{zhou2022crossview} uses a learned map embedding and an attention mechanism between map queries and camera features. In contrast to these existing BEV segmentation approaches that only use camera images, we explore the multi-modal fusion of LiDAR point clouds and camera images.\par

Multi-modal fusion for BEV segmentation has been enabled by recently introduced large-scale datasets providing time-synchronized data from multiple sensors~\cite{caesar2020nuscenes, geiger2013vision, sun2020waymo}. However, most works on these datasets focus on the 3D object detection task~\cite{klingner2023x, li2022deepfusion, liu2022bevfusion, yin2021center, chitta2022transfuser, shao2022safety}, while we focus on BEV segmentation. The closest prior art to our work is BEVFusion~\cite{liu2022bevfusion}. While their method also predicts BEV segmentation based on LiDAR point clouds and camera images, they use a simple feature concatenation to fuse multi-modal features such that the network implicitly has to connect information from misaligned features. In contrast, we explicitly enforce alignment between multi-modal features. Also, we enforce alignment between PV and BEV segmentation to improve the PV-to-BEV transformation.\par

\textbf{Camera-LiDAR Sensor Fusion}:
The vast majority of fusion methods have been proposed for the 3D object detection task. Initially, two-stage approaches have been proposed, lifting image bounding box proposals into 3D frustum view~\cite{nabati2021centerfusion, qi2018frustrum, wang2019frustum} for fusion with LiDAR. However, research focus has shifted towards end-to-end training, where approaches can roughly be divided into three categories: point-/input-level decoration, feature-level fusion, and proposal-level fusion. Point-level fusion includes methods such as PointAugmenting~\cite{wang2021pointaugmenting}, PointPainting~\cite{vora2020pointpainting}, FusionPainting~\cite{xu2021fusionpainting}, AutoAlign~\cite{chen2022autoalign}, and MVP~\cite{yin2021multimodal}, which extract camera features and use these features to enrich the point-level information, which is subsequently processed by a LiDAR-based detector. Recently proposed FocalSparseCNNs~\cite{chen2022focal} similarly enriches the features in the early feature extraction stage. For proposal-level fusion usually the predicted bounding boxes are refined~\cite{liang2022bevfusion}, often making use of an attention mechanism such as in FUTR3D~\cite{chen2022futr3d} and TransFusion~\cite{bai2022transfusion}. However, these two fusion types have downsides regarding generalization. While proposal-level fusion is not easily generalizable to other tasks, input-level decoration is not generically extendable to other sensor modalities.\par

Feature-level fusion aims at fusing extracted features from different sensors, subsequently predicting outputs for one or several tasks~\cite{li2022deepfusion, li2022bevformer, liang2018deep, liu2022bevfusion}. Our approach also falls into this category. While \cite{liang2018deep, liu2022bevfusion} use fusion via concatenation, more recent approaches apply attention-based fusion~\cite{li2022deepfusion, li2022bevformer}. However, these approaches still try to implicitly learn the interconnection between cross-modal features, while we explicitly encourage alignment between features from different modalities. Also, none of the above-mentioned methods uses attention-based cross-modal fusion for BEV segmentation or output-level segmentation alignment of PV and BEV segmentation.\par
%-------------------------------------------------

==> include/supp_arxiv_exps.tex <==
%-------------------------------------------------
\section{Varying Backbones}

%-------------------------------------------------
\input{tables/supp_backbones}
%-------------------------------------------------
To verify the generalizability of our X-Align method, we present results for three different encoders, \ie, SWin-T, ConvneXt-T, and ConvneXt-S, in Table~\ref{tab:backbones}. For this ablation study, we choose our \textbf{X-Align}$_{\mathrm{view}}$ variant because this shows that a given model can be improved without adding additional computational complexity during inference. Compared to the current state-of-the-art result from BEVFusion~\cite{liu2022bevfusion}, we can improve their result from 62.7 to 64.1 in terms of mIoU. Similar improvements can be observed for our additionally investigated backbones ConvneXt-T and ConvneXt-S. These results show that our method generalizes well to different backbones without hyperparameter tuning.
%-------------------------------------------------
\section{Adaptability to Noise}

%-------------------------------------------------
\input{tables/supp_noise}
%-------------------------------------------------

Another interesting property of deep neural network-based methods is their susceptibility to input perturbations because it gives insights into their robustness in real environments. Therefore, we add Gaussian noise to the input camera images and observe how the performance degrades in Table~\ref{tab:noise}.  The noise is zero-mean normalized, and $\sigma$ in Table~\ref{tab:noise} is the standard deviation of the Gaussian noise. From the table, we can deduce two main observations: First, the performance of X-Align methods under input perturbations is relatively stable compared to the baseline. We attribute this to the fact that the input camera noise will make the extracted camera feature less reliable. Due to our robust attention-based cross-modal feature fusion (X-FF), the method can still correct the camera features using LiDAR predictions. Our second interesting observation concerns the comparison to the baseline BEVFusion. We observe that our performance loss at a higher noise-variance is much smaller than for BEVFusion, e.g., the performance of our method \textbf{X-Align}$_{\mathrm{all}}$ at $\sigma=0.1$ drops from 65.7 to 59.6. In contrast, BEVFusion drops from 62.7 to 48.9. This shows superior properties of our method in terms of robustness.\par
%-------------------------------------------------
\section{Adverse Weather Conditions}

%-------------------------------------------------
\input{tables/supp_splits}
%-------------------------------------------------

To further investigate our method's robustness, we show results of how our method performs in adverse weather conditions in Table~\ref{tab:splits}. For this experiment, we use the metadata provided by nuScenes, which indicates the weather and light conditions of the recorded scene. With this information, we filter the validation set to obtain two splits containing all images recorded at night and all images recorded during rainy conditions. Our results show consistent improvement in these adverse conditions by \textbf{X-Align}$_{\mathrm{view}}$ as well as \textbf{X-Align}$_{\mathrm{all}}$. This shows that our method improves on comparably easy samples and difficult ones, which is an important property for future deployment of our method.
%-------------------------------------------------
\section{Training Details and Hyperparameter Analysis}

In this subsection, we provide the hyper-parameters and training details for all our experiments in the paper. All our models are trained using Pytorch~\cite{paszke2017automatic} on 4 Nvidia Tesla A100 GPUs.\par

\textbf{nuScenes experiments:} To reproduce the BEVFusion~\cite{liu2022bevfusion} baseline model, we adapt the code provided by their authors\footnote{\href{https://github.com/mit-han-lab/bevfusion}{https://github.com/mit-han-lab/bevfusion}} into the mmdetection3d~\cite{mmdet3d2020} framework. This is because they do not provide training code in the current version. In the camera pipeline, the images are downsampled into a size of $256\times704$ before being passed through a Swin-T~\cite{liu2021swin} or ConvNext~\cite{liu2022convnext} backbone pretrained on ImageNet~\cite{russakovsky2015imagenet}. The intermediate features extracted from the camera are passed through a set of FPN~\cite{lin2017feature} layers to retain the salient low-level encoder features. These are then passed to View-Transformers based on LSS~\cite{philion2020lift}. The baseline is trained using their reported hyper-parameters~\cite{liu2022bevfusion}, with a learning schedule of 20 epochs and a cyclic learning rate, starting for $1e^{-4}$ and performing a single cycle with target ratios $\{10, 1e^{-4}\}$ and a step of $0.4$. For our experiments, we implement our proposed blocks:
\begin{itemize}
\item
\textbf{X-FF Modules}: For the X-FF modules described in Section~3.3 of the paper, we switch the naive convolutional fuser in the baseline model. To implement the Self-Attention fuser, we tokenize the inputs into patches of size $3\times3$ and a stride of 2. This step is followed by a Multi-Head-Self-Attention block as described in~\cite{vaswani2017attention}, containing 8 heads and an embedding dimension of 256. To implement the Spatial-Channel Attention module, we use the Split-depth Transpose Attention (SDTA) block from EdgeNext~\cite{maaz2022edgenext}.We use an embedding dimension of 256, 2 scales, and 8 heads. We also use DropPath~\cite{larsson2016fractalnet} of $0.1$. A deconvolution block follows the SDTA fusion module to output 256 channels and the fused feature resolution. Finally, to implement the pose-driven deformable convolutional operation, we pass the input pose through a 2-layer MLP network, whose output can is interpolated to the feature size. This pose channel is concatenated with the two input modalities, then passes through a convolutional block to obtain $18$ offset channels, input into a DCNv2~\cite{zhu2019deformable} block of kernel size $3\times3$ The output of the DCNv2 block is our fused feature dimension.
\item
\textbf{X-FA Loss}: As explained in Section~3.4 of the paper, we use cosine similarity as a loss function to model the X-FA similarity. Using a sparse hyper-parameter search, we set the best value of $\gamma_{2}$ in Equation~(2) of the main paper as $-0.002$. We reduce its negative value because we want to increase the cosine similarity.
\item
\textbf{X-SA Module}: As explained in Section~3.5 of the paper, we utilize a perspective decoder to generate 2D perspective view semantic labels. The decoder has two Convolution-BN2D-ReLU sequences with a hidden dimension of $256$ channels, generating semantic probabilities at the output. As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels; we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase.\footnote{\href{https://github.com/Qualcomm-AI-research/InverseForm}{https://github.com/Qualcomm-AI-research/InverseForm}} We pick $\gamma_{3}$ in Equation~(2) of the main paper as $0.1$ following a sparse hyper-parameter search. Once we have the 2D perspective features, we share parameters with the LSS Transform from earlier to splat the probability maps to BEV space. We use convolution blocks for channel aggregation at the input and output and interpolate to equalize dimensions. The output is then supervised with BEV GT as shown in Figure~\ref{fig:method_detail1} of the paper. The loss weight $\gamma_4$ is tuned to $0.1$ by observing the total loss value and setting the weight to produce $\sim\! 20\%$ of the total loss. 
\end{itemize}

\textbf{KITTI360 experiments:} To reproduce the PanopticBEV~\cite{gosala22panopticbev} scores, we use the code made public by the authors and their default settings.\footnote{\href{https://github.com/robot-learning-freiburg/PanopticBEV}{https://github.com/robot-learning-freiburg/PanopticBEV}} The model consists of an EfficientDet-d3~\cite{tan2020efficientdet} camera encoder, which encodes multi-resolution features. Next, a multi-scale transformer converts the perspective view to BEV features. This is followed by decoders for both instance and semantics. Finally, their outputs are combined to generate panoptic predictions. The baseline uploaded by the authors reaches a lower value than what was obtained in their paper.  For our experiments with the \textbf{X-SA module}, we added a 2D Perspective decoder to the multi-scale encoded features to predict semantic labels in the perspective view. As KITTI360 contains 2d semantic labels, we use them to supervise this decoder. Then, we reuse the view transformer to map predictions to BEV space. We supervise our X-SA branch with loss weights $\gamma_3$ set at $0.5$ and $\gamma_4$ set at $0.1$, adding them to the total loss of the PanopticBEV baseline.

%As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels; we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase\footnote{https://github.com/Qualcomm-AI-research/InverseForm}.
%-------------------------------------------------
\section{Qualitative Analysis}

In this Section, we present more sample scenes from nuScenes, as an extension to the one shown in Figure~5 of the main paper. Each scene consists of 5 parts: a) six surround camera inputs b) LiDAR scan, c) ground-truth BEV segmentation map, d) baseline BEV segmentation, e) BEV segmentation using \textbf{X-Align}$_{\mathrm{view}}$, and d) BEV segmentation \textbf{X-Align}$_{\mathrm{all}}$. For each scenario, we observe that the baseline model prediction is highly erroneous in the region highlighted in \textcolor{green}{green}. We highlight this region of interest in the input views as well. By using our proposed X-SA losses, \textbf{X-Align}$_{\mathrm{view}}$ can already correct substantial errors in the baseline prediction, and the \textbf{X-Align}$_{\mathrm{all}}$ model further improves accuracy.

\input{figs/qualitative/supp_qualitative}
%-------------------------------------------------

==> include/supp_exps.tex <==
%-------------------------------------------------
\section{Varying Backbones}

%-------------------------------------------------
\input{tables/supp_backbones}
%-------------------------------------------------
To verify the generalizability of our X-Align method, we present results for three different encoders, \ie, SWin-T, ConvneXt-T, and ConvneXt-S, in Table~\ref{tab:backbones}. For this ablation study, we choose our \textbf{X-Align}$_{\mathrm{view}}$ variant because this shows that a given model can be improved without adding additional computational complexity during inference. Compared to the current state-of-the-art result from BEVFusion~\cite{liu2022bevfusion}, we can improve their result from 62.7 to 64.1 in terms of mIoU. Similar improvements can be observed for our additionally investigated backbones ConvneXt-T and ConvneXt-S. These results show that our method generalizes well to different backbones without hyperparameter tuning.
%-------------------------------------------------
\section{Adaptability to Noise}

%-------------------------------------------------
\input{tables/supp_noise}
%-------------------------------------------------

Another interesting property of deep neural network-based methods is their susceptibility to input perturbations because it gives insights into their robustness in real environments. Therefore, we add Gaussian noise to the input camera images and observe how the performance degrades in Table~\ref{tab:noise}.  The noise is zero-mean normalized, and $\sigma$ in Table~\ref{tab:noise} is the standard deviation of the Gaussian noise. From the table, we can deduce two main observations: First, the performance of X-Align methods under input perturbations is relatively stable compared to the baseline. We attribute this to the fact that the input camera noise will make the extracted camera feature less reliable. Due to our robust attention-based cross-modal feature fusion (X-FF), the method can still correct the camera features using LiDAR predictions. Our second interesting observation concerns the comparison to the baseline BEVFusion. We observe that our performance loss at a higher noise-variance is much smaller than for BEVFusion, e.g., the performance of our method \textbf{X-Align}$_{\mathrm{all}}$ at $\sigma=0.1$ drops from 65.7 to 59.6. In contrast, BEVFusion drops from 62.7 to 48.9. This shows superior properties of our method in terms of robustness.\par
%-------------------------------------------------
\section{Adverse Weather Conditions}

%-------------------------------------------------
\input{tables/supp_splits}
%-------------------------------------------------

To further investigate our method's robustness, we show results of how our method performs in adverse weather conditions in Table~\ref{tab:splits}. For this experiment, we use the metadata provided by nuScenes, which indicates the weather and light conditions of the recorded scene. With this information, we filter the validation set to obtain two splits containing all images recorded at night and all images recorded during rainy conditions. Our results show consistent improvement in these adverse conditions by \textbf{X-Align}$_{\mathrm{view}}$ as well as \textbf{X-Align}$_{\mathrm{all}}$. This shows that our method improves on comparably easy samples and difficult ones, which is an important property for future deployment of our method.
%-------------------------------------------------
\section{Training Details and Hyperparameter Analysis}

In this subsection, we provide the hyper-parameters and training details for all our experiments in the paper. All our models are trained using Pytorch~\cite{paszke2017automatic} on 4 Nvidia Tesla A100 GPUs.\par

\textbf{nuScenes experiments:} To reproduce the BEVFusion~\cite{liu2022bevfusion} baseline model, we adapt the code provided by their authors\footnote{\href{https://github.com/mit-han-lab/bevfusion}{https://github.com/mit-han-lab/bevfusion}} into the mmdetection3d~\cite{mmdet3d2020} framework. This is because they do not provide training code in the current version. In the camera pipeline, the images are downsampled into a size of $256\times704$ before being passed through a Swin-T~\cite{liu2021swin} or ConvNext~\cite{liu2022convnext} backbone pretrained on ImageNet~\cite{russakovsky2015imagenet}. The intermediate features extracted from the camera are passed through a set of FPN~\cite{lin2017feature} layers to retain the salient low-level encoder features. These are then passed to View-Transformers based on LSS~\cite{philion2020lift}. The baseline is trained using their reported hyper-parameters~\cite{liu2022bevfusion}, with a learning schedule of 20 epochs and a cyclic learning rate, starting for $1e^{-4}$ and performing a single cycle with target ratios $\{10, 1e^{-4}\}$ and a step of $0.4$. For our experiments, we implement our proposed blocks:
\begin{itemize}
\item
\textbf{X-FF Modules}: For the X-FF modules described in Section~\ref{sec:feature_fusion} of the paper, we switch the naive convolutional fuser in the baseline model. To implement the Self-Attention fuser, we tokenize the inputs into patches of size $3\times3$ and a stride of 2. This step is followed by a Multi-Head-Self-Attention block as described in~\cite{vaswani2017attention}, containing 8 heads and an embedding dimension of 256. To implement the Spatial-Channel Attention module, we use the Split-depth Transpose Attention (SDTA) block from EdgeNext~\cite{maaz2022edgenext}.We use an embedding dimension of 256, 2 scales, and 8 heads. We also use DropPath~\cite{larsson2016fractalnet} of $0.1$. A deconvolution block follows the SDTA fusion module to output 256 channels and the fused feature resolution. Finally, to implement the pose-driven deformable convolutional operation, we pass the input pose through a 2-layer MLP network, whose output can is interpolated to the feature size. This pose channel is concatenated with the two input modalities, then passes through a convolutional block to obtain $18$ offset channels, input into a DCNv2~\cite{zhu2019deformable} block of kernel size $3\times3$ The output of the DCNv2 block is our fused feature dimension.
\item
\textbf{X-FA Loss}: As explained in Section~\ref{sec:feature_alignment} of the paper, we use cosine similarity as a loss function to model the X-FA similarity. Using a sparse hyper-parameter search, we set the best value of $\gamma_{2}$ in Equation~(\ref{eq:final_loss}) of the main paper as $-0.002$. We reduce its negative value because we want to increase the cosine similarity.
\item
\textbf{X-SA Module}: As explained in Section~\ref{sec:segmentation_alignment} of the paper, we utilize a perspective decoder to generate 2D perspective view semantic labels. The decoder has two Convolution-BN2D-ReLU sequences with a hidden dimension of $256$ channels, generating semantic probabilities at the output. As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels; we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase.\footnote{\href{https://github.com/Qualcomm-AI-research/InverseForm}{https://github.com/Qualcomm-AI-research/InverseForm}} We pick $\gamma_{3}$ in Equation~(\ref{eq:final_loss}) of the main paper as $0.1$ following a sparse hyper-parameter search. Once we have the 2D perspective features, we share parameters with the LSS Transform from earlier to splat the probability maps to BEV space. We use convolution blocks for channel aggregation at the input and output and interpolate to equalize dimensions. The output is then supervised with BEV GT as shown in Figure~\ref{fig:method_detail1} of the paper. The loss weight $\gamma_4$ is tuned to $0.1$ by observing the total loss value and setting the weight to produce $\sim\! 20\%$ of the total loss. 
\end{itemize}

\textbf{KITTI360 experiments:} To reproduce the PanopticBEV~\cite{gosala22panopticbev} scores, we use the code made public by the authors and their default settings.\footnote{\href{https://github.com/robot-learning-freiburg/PanopticBEV}{https://github.com/robot-learning-freiburg/PanopticBEV}} The model consists of an EfficientDet-d3~\cite{tan2020efficientdet} camera encoder, which encodes multi-resolution features. Next, a multi-scale transformer converts the perspective view to BEV features. This is followed by decoders for both instance and semantics. Finally, their outputs are combined to generate panoptic predictions. The baseline uploaded by the authors reaches a lower value than what was obtained in their paper.  For our experiments with the \textbf{X-SA module}, we added a 2D Perspective decoder to the multi-scale encoded features to predict semantic labels in the perspective view. As KITTI360 contains 2d semantic labels, we use them to supervise this decoder. Then, we reuse the view transformer to map predictions to BEV space. We supervise our X-SA branch with loss weights $\gamma_3$ set at $0.5$ and $\gamma_4$ set at $0.1$, adding them to the total loss of the PanopticBEV baseline.

%As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels; we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase\footnote{https://github.com/Qualcomm-AI-research/InverseForm}.
%-------------------------------------------------
\section{Qualitative Analysis}

In this Section, we present more sample scenes from nuScenes, as an extension to the one shown in Figure~\ref{fig:qualitative} of the main paper. Each scene consists of 5 parts: a) six surround camera inputs b) LiDAR scan, c) ground-truth BEV segmentation map, d) baseline BEV segmentation, e) BEV segmentation using \textbf{X-Align}$_{\mathrm{view}}$, and d) BEV segmentation \textbf{X-Align}$_{\mathrm{all}}$. For each scenario, we observe that the baseline model prediction is highly erroneous in the region highlighted in \textcolor{green}{green}. We highlight this region of interest in the input views as well. By using our proposed X-SA losses, \textbf{X-Align}$_{\mathrm{view}}$ can already correct substantial errors in the baseline prediction, and the \textbf{X-Align}$_{\mathrm{all}}$ model further improves accuracy.
%-------------------------------------------------
\input{figs/qualitative/supp_qualitative}
%-------------------------------------------------

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


